Towards Using Promises for Multi-Agent Cooperation in Goal Reasoning

Reasoning and planning for mobile robots is a challenging problem, as the world evolves over time and thus the robot's goals may change. One technique to tackle this problem is goal reasoning, where the agent not only reasons about its actions, but also about which goals to pursue. While goal reasoning for single agents has been researched extensively, distributed, multi-agent goal reasoning comes with additional challenges, especially in a distributed setting. In such a context, some form of coordination is necessary to allow for cooperative behavior. Previous goal reasoning approaches share the agent's world model with the other agents, which already enables basic cooperation. However, the agent's goals, and thus its intentions, are typically not shared. In this paper, we present a method to tackle this limitation. Extending an existing goal reasoning framework, we propose enabling cooperative behavior between multiple agents through promises, where an agent may promise that certain facts will be true at some point in the future. Sharing these promises allows other agents to not only consider the current state of the world, but also the intentions of other agents when deciding on which goal to pursue next. We describe how promises can be incorporated into the goal life cycle, a commonly used goal refinement mechanism. We then show how promises can be used when planning for a particular goal by connecting them to timed initial literals (TILs) from PDDL planning. Finally, we evaluate our prototypical implementation in a simplified logistics scenario.

==> pddl.tex <==
\lstdefinelanguage{PDDL}{
  keywordsprefix=?,
  %keywordsprefix=\$,
  alsoletter={?=-<>*\$:},
  alsodigit={:},
  keywordstyle=\color{rwth-blue},
  keywords=[2]{define, domain, problem, :requirements, :predicates,
    :types, :objects, :action, :init, :goal, :domain, :constants},
  keywords=[3]{ :parameters, :vars, :precondition, :effect },
  keywords=[4]{ forall, or, and, not, when, =, exists, imply },
  keywords=[5]{
    :strips,
    :typing,
    :negative-preconditions,
    :disjunctive-preconditions,
    :equality,
    :existential-preconditions,
    :universal-preconditions,
    :quantified-preconditions,
    :conditional-effects,
    :fluents,
    :numeric-fluents,
    :adl,
    :durative-actions,
    :duration-inequalities,
    :continuous-effects,
    :derived-predicates,
    :timed-initial-literals,
    :preferences,
    :constraints,
    :action-costs},
  keywordstyle=[2]\color{rwth-red!70!black}\bfseries,
  keywordstyle=[3]\color{gray!80}\bfseries,
  keywordstyle=[4]\color{darkgray!80}\bfseries,
  keywordstyle=[5]\color{Mulberry},
  %identifierstyle=\color{black},
  sensitive=false,
  comment=[l]{;},
  commentstyle=\color{purple}\ttfamily,
  stringstyle=\color{red}\ttfamily,
  morestring=[b]"
}


\lstdefinestyle{PDDLNoFloat}
{
  language=PDDL,
  basicstyle=\footnotesize\ttfamily\vspace{0.2cm},
  breaklines=true,
  showstringspaces=false,
  %keywordstyle=\bfseries,
  %keywordstyle=\color{Mulberry},
  frame=lines,
  emphstyle=\color{orange!70!black}\itshape,
  numbers=none,
  %stepnumber=1,
  backgroundcolor=\color{gray!5},
  rulecolor=\color{gray!80},
  %fillcolor=\color{blue!20},
  framexleftmargin=0pt,
  xleftmargin=0pt,
  %stringstyle=\color{BitterSweet},
  stringstyle=\color{BrickRed},
  commentstyle=\color{BrickRed},
  escapechar=\%,
  % emph={getup, servo, depends_skills},
  %emphstyle=\underbar,
  %numbers=left,
  %stepnumber=1,
  %%stringstyle=\ttfamily, % typewriter type for strings
}

\lstdefinestyle{PDDL}
{
  style=PDDLNoFloat,
  float,
  numbers=left,
  framexleftmargin=16pt,
  xleftmargin=16pt,
  captionpos=b,
  belowcaptionskip=-8pt,
  %belowskip=0pt
}

\lstdefinestyle{SmallPDDL}{
  style=PDDL,
  basicstyle=\ttfamily\footnotesize,
  numbersep=6pt,
}
\lstdefinestyle{ReallySmallPDDL}{
  style=PDDL,
  basicstyle=\ttfamily\scriptsize,
  numbersep=5pt,
}

\lstdefinestyle{ReallySmallPDDLNoNumbers}{
  style=ReallySmallPDDL,
  xleftmargin=0pt,
  numbers=none,
  framexleftmargin=0pt,
}

\lstdefinestyle{ReallySmallPDDLNoFrame}{
  style=PDDL,
  basicstyle=\ttfamily\scriptsize,
  numbersep=5pt,
  frame=none,
  backgroundcolor=\color{white},
  framextopmargin=0pt,
  framexbottommargin=0pt
}

\lstdefinestyle{SmallPDDLNoFrame}{
  style=PDDL,
  basicstyle=\ttfamily\footnotesize,
  numbersep=5pt,
  frame=none,
  backgroundcolor=\color{white},
  framextopmargin=0pt,
  framexbottommargin=0pt
}

\lstdefinestyle{SmallPDDLNoFloat}{
  style=PDDLNoFloat,
  basicstyle=\ttfamily\footnotesize,
  numbersep=6pt,
}

